Polylogarithmic Approximation Algorithm for k-Connected Directed Steiner Tree on Quasi-Bipartite Graphs

In the k-Connected Directed Steiner Tree problem (k-DST), we are given a directed graph G=(V, E) with edge (or vertex) costs, a root vertex r, a set of q terminals T, and a connectivity requirement k>0; the goal is to find a minimum-cost subgraph H of G such that H has k internally disjoint paths from the root r to each terminal t . The k-DST problem is a natural generalization of the classical Directed Steiner Tree problem (DST) in the fault-tolerant setting in which the solution subgraph is required to have an r,t-path, for every terminal t, even after removing k-1 edges or vertices. Despite being a classical problem, there are not many positive results on the problem, especially for the case k >= 3. In this paper, we will present an O(log k log q)-approximation algorithm for k-DST when an input graph is quasi-bipartite, i.e., when there is no edge joining two non-terminal vertices. To the best of our knowledge, our algorithm is the only known non-trivial approximation algorithm for k-DST, for k >= 3, that runs in polynomial-time regardless of the structure of the optimal solution. In addition, our algorithm is tight for every constant k, due to the hardness result inherited from the Set Cover problem.

==> facility.tex <==
\section{The Main Subroutine: Covering Halo-Families}
\label{sec:covering-halo-families}
% An approximation algorithm for k-directed Steiner tree on the quasi-bipartite graph shows as Algorithm 1. 
% The main results is to show that Algorithm 1 with approximation ratio $O(\log k~\log^2q)$.
% It is a stander result to show that the losing of $O(\log k)$ factor of the augmentation from $k-1$ to $k$.
% Thus, it is remain to show the we can have a $O(\log^2 q)$ algorithm for the augmentation subroutine.

% We shows that the algorithm will recursively process $O(log n)$ rounds in each augmentation subroutine.
% In each round, the Halo family of each existing core can be computed,
% and we greedily cover those deficient sets in each Halo families by mapping the Cover Problem to the Facility Location Problem.
% While finding the solution in the Facility Location Problem,
% we can apply a corresponding mapping to find a feasible solution in the Cover Problem.
In this section, we present our subroutine for covering the Halo-families that arose from the Rooted-Aug problem. The main ingredient is a reduction from the problem of covering Halo-families to the facility location problem, which exploits the structure of quasi-bipartite graphs.
%We construct a Related Facility Location Problem and use the result of the Facility Location Problem to choose the new edge set $\Delta_E$. Before that, we first give the formal definition of Facility Location problem we use in this section.
Please recall to the definition of the Facility Location problem in \Cref{sec:prelim:problem}.

%\begin{definition}[the Facility Location Problem]

%Given a set of facilities $P = \{p_1,p_2...p_n\}$ and a set of centers $D = \{D_1, D_2...D_m\}$. Each facility has a open cost $c_{i}$, $\forall i\in P$ and each client has a distance $D_{ij}$, $\forall i\in P, j\in D$. Our goal is to open a set of facilities $P^{\ast}$ which every center can be served and minimized the total cost. 

%\end{definition}

To ease, the presentation, we need to define some terminologies, and some graph terminologies will be abused.

\begin{definition}[In-coming edge]
An {\em in-coming edge} of a vertex set $S$ is an edge $(u,v)$ where $v\in S$ and $u\in V\setminus S$.
We use $\En(S)$ to denote the set of in-coming edges of a set $S$.
\end{definition}

\begin{definition}[Inside edge]
An {\em inside edge} of a vertex set $S$ is an edge $(u,v)$ where both endpoints $u,v$ are in $S$.
The set of inside edges of a set $S$ is denoted by $\Em(S)$.
\end{definition}

\begin{definition}[Inside Cost]
Given a pair $(C,e)$, where $C$ is a core and $e$ is an edge $e$ incoming to the Halo-family $\Halo(C)$, the {\em inside-cost} for covering the Halo Family $\Halo(C)$ is the minimum cost subset of inside-edges that covers all the deficient sets in $\Halo(C)$ while using only the inside-edges in $\Em(S)$ and the edge $e$ (i.e., $e$ is the only edge incoming to $\Halo(C)$). If there exists no subset of edges $E'\subseteq \Em(S)\cup\{e\}$ that covers $\Halo(C)$, then the inside-cost is defined to be the total cost of all the edges in $E(G)$.
\end{definition}

The set of edges corresponding to the inside-cost is denoted by $\IC(C,e)$. For the case, that the inside-cost is infinity we may define $\IC(C,e)$ as the set of edges of the entire graph; that is,
$$
\IC(C,e) = \text{argmin}\left\{\{\cost(E): E'\subseteq \Em(S) \land E'\cup\{e\} \text{ covers } \Halo(C)\}\cup \{\cost(E(G))\}\right\}.
$$

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{definition_example.png}
    \caption{Example of the definitions.}
    \label{fig:s5definition}
\end{figure}

We give a picture for these definition in Figure~\ref{fig:s5definition}. It's a Halo family $\Halo(C)$ contains the deficient set $C, U_1,U_2$ and $U_3$,where C is the core of such Halo family $\Halo(C)$. The edges $e_1$ and $e_2$ are the in-coming edges of the Halo set $H(C)$. The edges $e_3$, $e_4$, and $e_5$ are the inside edges of the Halo set $H(C)$. The inside cost $IC(C,e_1)=\{ e_4, e_5\}$, $IC(C,e_2)=\{e_3,e_4\}$.

The next lemma shows that $\IC(C,e)$ can be computed in polynomial-time. 

\begin{lemma}
For any core $C$ and an edge $e$ incoming to $\Halo(C)$, the inside-cost $\cost(IC(C,e))$ can be computed in polynomial-time. Moreover, the standard LP for computing $\IC(C,e)$ is integral.
\end{lemma}
\begin{proof}
Consider the Halo-family $\Halo(C)$.
Observe that, for any deficient sets $U,W\in\Halo(C)$, both $U\cap W$ and $U\cup W$ must be deficient sets in $\Halo(C)$. This is because both $U$ and $W$ contain $C$ and thus have a non-empty intersection on the terminal set. In addition, $U\cup W$ contains no core $C'\neq C$; otherwise, at least one of $U$ and $W$ must contain a terminal in $C'$, which is a contradiction since $C$ and $C'$ have no common terminal.
%
Consequently, $\Halo(C)$ is an {\em intersecting family}, which implies that its standard LP (i.e., $\LP^{aug}(\ell)$ where $\mathcal{F}(\ell)=Halo(C)$) is integral. 
%
Alternatively, we may compute $\IC(C,e)$ combinatorially using a minimum-cost $(\ell+1)$-flow algorithm. In particular, we construct and $s^*,t^*$-flow network by setting the costs of the edges in $E(G_0)\cup\{e\}$ to zero, adding a source $s^*$ connecting to $\ell+1$ edges entering $\Halo(C)$ (which consists of $\ell$ edges from $\delta^{+}_{G_0}(U)$ and the edge $e$) and then picking an arbitrary terminal $t^*\in C$ as a sink; all the edges outside $\Halo(C)$ except $\delta^{+}_{G_0}(U)\cup \{e\}$ are removed. 
In this $s,t$-flow network, if there exists a feasible solution for the problem of covering $\Halo(C)$, then Menger's theorem implies that there must exist an $(\ell+1)$-flow from $s^*$ to $t^*$ with the same cost. It is not hard to see that the minimum-cost over all $(\ell+1)$-flows yields a minimum-cost cover of $\Halo(C)$ and vise versa. 
\end{proof}

\subsection{Reduction to Facility Location}
\label{sec:covering-halo-families:reduction-to-FLP}

As mentioned, the key ingredient in our algorithm is the reduction from the problem of covering Halo-families to the Facility Location problem. Here we show a reduction from the problem of cover Halo-families to an instance of the Facility Location problem.
Please see \Cref{algo_2} for details.

Let $\mathcal{C}$ be the set of cores of the current solution subgraph. We construct an instance of the Facility Location problem by first defining each core $C\in\mathcal{C}$ as a client $D_C$ and then defining each edge $e$ as a facility $P_e$. The openning cost of a facility $P_e$ is $p(P_e) = c_e$ (i.e., the same as the cost of $e$), and the cost for connecting $P_e$ to a client $D_C$ is $\dist(C,e)=\cost(\IC(C,e))$. We denote this instance of the Facility Location problem by $\phi_{FL}$ and denote the cost of its optimal solution by $\opt_{FL}$.

%The key approach we use is that we try to cover every single Halo-Family by an "In-coming Edge, Inside Cost" pair. We further let the in-coming edge to be a facility and the the related Inside Cost to be the distance to construct the Related Facility Location Problem, we also show the whole steps in Algorithm~\ref{algo_2}.

%\paragraph*{Related Facility Location Problem:RFLP}
%Given every core $C$ and every in-coming edge $e$ of the Halo set $H(C)$
%We define the center, facility cost, and distance as follows:
%\begin{enumerate}
%\item Let every core $C$ be a center $D_C$ of the facility location problem.
%\item For every in-coming edge $e$ which $cover$ the Halo set $H(C)$, let $e$ be a facility $P_e$ (The cost of the facility is equal to cost of the edge $e$).
%\item The distance $dis(P_e,D_C)$ between a center $D_C$ and a facility $P_e$ is equal to $Cost(IC(C,e))$ if $E'_c(Halo(C),e)$ exists, otherwise, $dis(P_e,D_C)=\infty$.
%\end{enumerate}

%\paragraph*{Choose $\Delta_E$ based on the RFLP}
%$\Delta_E$ is the new edge set chosen in this round based the given solution of the Related Facility Location Problem. That is, 
%\begin{enumerate}
%\item Add all $e$ related to the opened facility to $\Delta_E$.
%\item For every core, it has to pay a minimum distance $dis(C,e)$, add the related $IC(C,e)$ to $\Delta_E$
%\end{enumerate}
Let $\opt_{cover}$ be the cost of the minimum-cost subset of edges that covers all the Halo-families.
Then it is easy to see that $\opt_{cover} \leq \opt_{FL}$.
\begin{lemma}
$\opt_{cover} \leq \opt_{FL}$.
\end{lemma}

\begin{algorithm}[ht]
\begin{algorithmic}[1]
\caption{\hspace{-1mm}: Algorithm for Halo Family Cover Problem }\label{algo_2}
\Require: A collection of cores $\mathcal{C}$ and their Halo-Set $H(C)$ for $C\in\mathcal{C}$.
\Ensure: An edge Set $E'$ that covers all $\Halo(C)$.
\State Construct an instance of $\phi_{FLP}$ of the Facility Location problem.
\State Approximate $\phi_{FLP}$.
\State Return the set of edges $E'$ corresponding to the solution to $\phi_{FLP}$.
\end{algorithmic}
\end{algorithm}

It is well-known that there exists an $O(\log q)$ approximation algorithm to the Facility Location problem, which can be either a combinatorial algorithm or LP-based; see, e.g., \cite{Hochbaum82}. Thus, to complete the proof, we need to bound the optimal solution to $\opt_{FL}$ with $\opt_{cover}$. To do so, first, we show that, for every core $C$, $\opt_{cover}$ has to pay at least the cost of  $\IC(C,e)$ for some incoming edge $e$. Furthermore, we argue that any two cores cannot share inside edges, which follows from the property of quasi-bipartite graphs. Thus, roughly saying, what $\opt_{cover}$ can do is similarly to the Facility Location problem. 

\begin{lemma}
\label{lem:optbound}
For all core $C$, there exist an in-coming edge $e$, such that $IC'(C) \cup {e} \subset \opt_k$ where $IC'(C)$ is a set of inside edges of $H(C)$ and $cost(IC'(C))\geq cost(IC(C,e))$.
\end{lemma}
\begin{proof}
We first pick up all in-coming edges of $H(C)$ chosen in $\opt_k$, let's say $E_A$. $E_A = \opt_k \cap \En(H(C))$ cannot be $\emptyset$ because $\opt_k$ should cover all deficient set in \Halo(C). Then we further collect all inside edge of $H(C)$ chosen in $\opt_k$ to be $E_B = \opt_k \cap \Em(H(C))$. After that, we find a minimal subset $E_C \subset E_A$ such that $E_C \cup E_B$ can still cover all deficient sets in $\Halo(C)$. We prove that $|E_C| = 1$, otherwise, we can find several in-coming edges $e_1$ and $e_2$, which should be used to cover several different deficient sets. Let them be $U_1,U_2,...,U_l$, which are deficient set which are not covered if by $E_C-\{e1,e2\} \cup E_B$. By \cref{lem:uncrossing}, $\bigcap_{i=1}^{l} U_i$ should also be a deficient set because it contains the core, we must have an edge $e_3 = (u,v) \in E_C \cup E_B$, If $e_3 \in E_C$, then we got that $E_C-\{e_1,e_2\}\cup \{e_3\} \cup E_B$ can cover the whole Halo Family, which means we can remove at least one of $e_1,e_2$ from $E_C$ and $E_C \cup E_B$ is still a cover. While if $e_3 \in E_B = (u,v)$, then we have that all the deficient set not contain $u \notin \bigcap_{i=1}^{l} U_i$ can be covered by $E_C-\{e1,e2\} \cup E_B$, we remove these $U_i$, and keep the other $U$ set to repeat find another $e_3$. Finally, the progress will stop at finding an $e_3$ which is an In-Coming Edge so that we can at least remove one of $e_1$ and $e_2$ and after that $E_C\cup E_B$ can still cover all deficient set in $\Halo(C)$. (We give an example in Figure~\ref{fig:minimal}. Thus, we can find a set $IC'(C) \cup {e}\subset \opt_k$ which can cover all deficient sets in $\Halo(C)$. Finally, for that $IC(C,e)$ is the minimum solution to cover $\Halo(C)$ by using only one in-coming edge $e$, we can find $IC'(C)\cup {e} \subset \opt_k$, $\cost(IC'(C))\geq \cost(IC(C,e))$.   
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=0.3\paperwidth]{minimal.png}
    \caption{Step 1: $U_1,U_2,U_3$ find $e_3$. Step 2: $U_1,U_2$, find $e_3'$. Step 3: $U_1$, find $e_1$, keep $e_1$, remove $e_2$.}.
    \label{fig:minimal}
\end{figure}

\begin{lemma} 
In each round, $\opt_{FL} \leq 2\opt_k$.
\end{lemma}
\begin{proof}
Let's say in this round, there are $l$ cores $C_1,C_2,...,C_l$.
From Lemma \ref{lem:optbound}, for every core $C_i$, we can find an edge $e_i$, such that $\opt_{cover}$ includes a subset $IC'(C_i)\cup{e_i}$.
Then we construct a feasible solution of the Facility Location problem, let's say \textsf{FL}, and we prove its cost is at most $2\opt_{cover}$: \\
For every $i\in[l]$, if $\opt_{cover}$ chooses $IC'(C_i)\cup{e_i}$, then open the facility $P_{e_i}$ (if it has not been open yet). Thus, The feasible solution has cost $$\cost(\textsf{FL}) \leq \cost (\bigcup_{i=1}^{l}{e_i})  + \sum_{i=1}^{l} {\cost(IC(C_i,e_i))} \leq \cost (\bigcup_{i=1}^{l}{e_i}) + \sum_{i=1}^{l} \cost(IC'(C_i)).
$$ 

Note, however, in $\opt_{cover}$ we have:
$$\opt_{cover} \geq \cost(\bigcup_{i=1}^{l} IC'(C_i)\cup{e_i})$$. 
By \Cref{lem:inside-disjoint}, for two cores $C'$and $C''$, $\En(H(C')) \cap \En(H(C'') = \emptyset$ so that $\sum_{i=1}^{l} \cost(IC'(C_i)) = \cost(\bigcup_{i=1}^{l} IC'(C_i))$. Thus, we only double count the edges if they appear as inside-edges of some Halo-family, while appearing as Inside-Edges of another Halo-family (which they can be in only one of them). Please see \Cref{fig:FLPcost} for illustration. This shows that $\cost(\textsf{FL}) \leq 2 \opt_k$, which proves the Lemma.

\begin{figure}
    \centering
    \includegraphics[width=0.3\paperwidth]  {2OPT.PNG}
    \caption{$e_3$ is the Inside Edge of $\Halo(C_1)$, and also an In-Coming Edge of $\Halo(C_2)$.}
    \label{fig:FLPcost}
\end{figure}

\end{proof}

\begin{corollary}
$\cost(E') \leq O(\log q) \opt_{FL} \leq O(\log q) \opt_{cover} \leq O(\log q) \opt_{aug}$,
where $\opt_{aug}$ is the cost of the optimal solution to the rooted-connectivity augmentation problem.
\end{corollary}
\begin{proof}
By the result shown in \cite{Hochbaum82}, Greedy algorithm can give a $O(\log q)$ approximate result of Facility Location problem, this lemma just complete the proof of Lemma~\ref{lem:HFCmain}.
\end{proof}

\begin{lemma}
\label{lem:inside-disjoint}
Given two distinct cores $C$and $C'$, we know that $\En(H(C)) \cap \En(H(C') = \emptyset$.
\end{lemma}

\begin{proof}
This statement is proved by a contradiction.
Consider two distinct cores $C$ and $C'$.
Suppose that $\En(H(C)) \cap \En(H(C')\neq\emptyset$.
Then there must exist an edge $(u,v)$, where both $u, v\in\En(H(C))\cap\En(H(C')$.
Furthermore, for any vertex $v\in\En(H(C))\cap\En(H(C')$, $v$ cannot be a terminal vertex by \Cref{lem:terminal-disjoint}
because, otherwise, it would contradict the definition of deficient sets.
Thus, both $u, v$ are the Steiner vertices.
But, then this contradicts the definition of the quasi-bipartite graph.
\end{proof}
